Quantifying Uncertainty in Natural Language Explanations of Large Language Models

Large Language Models (LLMs) are increasingly used as powerful tools for several high-stakes natural language processing (NLP) applications. Recent prompting works claim to elicit intermediate reasoning steps and key tokens that serve as proxy explanations for LLM predictions. However, there is no certainty whether these explanations are reliable and reflect the LLMs behavior. In this work, we make one of the first attempts at quantifying the uncertainty in explanations of LLMs. To this end, we propose two novel metrics -- $\textit{Verbalized Uncertainty}$ and $\textit{Probing Uncertainty}$ -- to quantify the uncertainty of generated explanations. While verbalized uncertainty involves prompting the LLM to express its confidence in its explanations, probing uncertainty leverages sample and model perturbations as a means to quantify the uncertainty. Our empirical analysis of benchmark datasets reveals that verbalized uncertainty is not a reliable estimate of explanation confidence. Further, we show that the probing uncertainty estimates are correlated with the faithfulness of an explanation, with lower uncertainty corresponding to explanations with higher faithfulness. Our study provides insights into the challenges and opportunities of quantifying uncertainty in LLM explanations, contributing to the broader discussion of the trustworthiness of foundation models.

==> aistats2024/020related.tex <==
\section{Related works}
\label{sec:related}
Our work lies at the intersection of large language models, explainability, and uncertainty estimation, which we discuss below.

\looseness=-1 \xhdr{Large Language Models} In the field of natural language processing (NLP), Large Language Models (LLMs) have proven their efficacy in various tasks, including sentiment analysis, text summarization, and machine translation. Moreover, they have become the backbone of modern conversational agents and virtual assistants, powering chatbots like GPT-3 \cite{NEURIPS2020_1457c0d6}, GPT-4 \cite{bubeck2023sparks}, Llama-2 \cite{touvron2023llama}, and Claude \cite{claudeanthropic} that offer human-like interactions. \citet{kaddour2023challenges} provide a survey of the applications of LLMs in Chatbots, Computational Biology, Creative Work, Knowledge Work, Law, Medicine, Reasoning, Robotics, Social Sciences, and Synthetic Data Generation. While the adaptability of LLMs to a wide array of applications underscores their potential to reshape industries through enhanced natural language understanding, there exists a gap in trusting these models and deploying them to real-world users.

\looseness=-1 \xhdr{Explainability} Explainability in machine learning has gained significant attention as the deployment of complex models has become more pervasive in critical applications. The need for understanding model decisions and gaining insights into their inner workings has led to the development of various explainability techniques.  While there have been a plethora of perturbation-based, gradient-based, example-based, and surrogate-based methods, none of these explanation methods are feasible for LLMs as they require some level of model access, \eg gradients or logits. Chain-of-Thought (CoT) explanations~\citep{wei2023chainofthought}, a form of natural language explanation generated by prompting LLMs, are the state-of-the-art alternative for models without open-source access and has shown to provide plausible and human-interpretable reasoning behind LLM predictions. However, several questions have been raised about the reliability of these explanations.
% \citet{lanham2023measuring} quantifies the faithfulness of Chain-Of-Thought explanations at a dataset level by intervening in explanations.
% \chirag{Editing here}
% Feature attribution methods aim to identify the importance of input features in the model's predictions. Common approaches include perturbation-based methods, gradient-based methods, and surrogate models. Perturbation-based methods like Integrated Gradients compute feature importance by perturbing input features and observing their impact on predictions. Gradient-based methods, exemplified by Gradient*Input, compute feature importance using gradients of model outputs with respect to input features. Surrogate models, such as LIME (Local Interpretable Model-agnostic Explanations), provide interpretable approximations of complex models' behavior. 
% Example-based methods focus on generating instances that highlight model behavior. Counterfactuals create instances that result in different model predictions while closely resembling the original input. Adversarial examples are crafted to perturb inputs minimally to mislead the model. These techniques help reveal model sensitivities and decision boundaries.
% Attention mechanisms, initially popularized in sequence-to-sequence models (Bahdanau et al., 2015), have been adapted for explainability purposes. Attention maps visualize the model's focus on different parts of the input during inference. Recent work in interpretability extends attention-based methods to vision and language models (e.g., Vision Transformers and BERT) (Carion et al., 2020; Devlin et al., 2018). These methods offer insights into what the model pays attention to when making predictions.
% However, none of the aforementioned explanation methods are feasible for black box language models. Natural language explanation methods generated by prompting the model is the only alternative for models without open source access. Chain-Of-Thought Explanations have shown to provide plausible and human interpretable reasoning behind LLM predictions. However, several questions have been raised about whether these natural language explanations are faithful. \cite{lanham2023measuring} quantifies the faithfulness of Chain-Of-Thought explanations at a dataset level by intervening on explanations.

\looseness=-1\xhdr{Uncertainty Estimation} Traditional ways to measure the confidence of predictions primarily rely on model logits, have become less suitable for LLMs and even infeasible with the development of closed-source LLMs. While \citet{xiong2023llms} proposes approaches for confidence elicitation of black-box LLMs, to the best of our knowledge, our work is the first to tackle the problem of estimating the uncertainty in NLEs.
% are the first no other work has specifically tackled the problem we are working on, i.e; estimating the uncertainty of natural language explanations.
% Reliable uncertainty estimates of generated text are crucial for human-machine collaboration, and rational decision making. 
